A Discrete Variational Recurrent Topic Model without the Reparametrization Trick

We show how to learn a neural topic model with discrete random variables---one that explicitly models each word's assigned topic---using neural variational inference that does not rely on stochastic backpropagation to handle the discrete variables. The model we utilize combines the expressive power of neural methods for representing sequences of text with the topic model's ability to capture global, thematic coherence. Using neural variational inference, we show improved perplexity and document understanding across multiple corpora. We examine the effect of prior parameters both on the model and variational parameters and demonstrate how our approach can compete and surpass a popular topic model implementation on an automatic measure of topic quality.

==> generated-sentences-short.tex <==
\begin{table*}
    \centering
    \resizebox{.98\textwidth}{!}{
    \begin{tabular}{c|l}
    \specialrule{.1em}{.1em}{-0.01em}
    \multicolumn{1}{l|}{\textbf{Data}}                    & \multicolumn{1}{c}{\textbf{Generated Sentences}}                                                       \\ \hline
    \multicolumn{1}{l|}{\multirow{8}{*}{\textbf{APNEWS}}} & $\bullet$  a damaged car and body $<$unk$>$ were taken to the county medical center from dinner with one driver.\\
    \multicolumn{1}{l|}{}                        & $\bullet$  the house now has released the $<$unk$>$ of \$ 100,000 to former $<$unk$>$ freedom u.s. postal service \\
    \multicolumn{1}{l|}{}                        & \ \ \ \ \ \ and \$ $<$unk$>$ to the federal government. \\
    % \multicolumn{1}{l|}{}                        & $\bullet$  that senate passed both chambers and filed a similar approval friday . under the 2007 law . \\
   % \multicolumn{1}{l|}{}                        & $\bullet$  the man was able to cross the river and was pronounced dead at a hospital .  \\
    \multicolumn{1}{l|}{}                        & $\bullet$  another agency will investigate possible abuse of violations to the police facility .\\
    \multicolumn{1}{l|}{}                        & $\bullet$  not even if it represents everyone under control . we are getting working with other items .\\
    \multicolumn{1}{l|}{}                        & $\bullet$  the oklahoma supreme court also faces a maximum amount of money for a local counties.\\
    \multicolumn{1}{l|}{}                        & $\bullet$  the money had been provided by local workers over how much $<$unk$>$ was seen in the spring. \\
    %\multicolumn{1}{l|}{}                        & $\bullet$  the independent newspaper reports davis said she thinks the library had no choice because she 's considering either enter a u.s. \\ & \quad constitution under u.s. senate action .\\
    \multicolumn{1}{l|}{}                        & $\bullet$  he did n't offer any evidence and they say he was taken from a home in front of a vehicle.\\ 
    % \multicolumn{1}{l|}{}                        & $\bullet$  the most violent $<$unk$>$ has since left the courtroom , marking the final day of the debate this week in california.  \\
    %\multicolumn{1}{l|}{}                        & $\bullet$  two towns at the holy least seven square miles south of nebraska.\\ 
    \hline
    % \multicolumn{1}{l|}{}                        & $\bullet$  since then , in its announcement on thursday , the meeting is likely to be presented with chicago .\\
    % \multicolumn{1}{l|}{}                        & $\bullet$  the oregonian reports about $<$unk$>$ children were hiking about $<$unk$>$ p.m. throughout the 2013 \\&\quad creek city of $<$unk$>$ on dec. 29 \\ \hline
    \specialrule{.1em}{.05em}{.05em}
    \end{tabular}
    }
    \caption{Seven randomly generated sentences from a VRTM model learned on the APNEWS corpus. See \cref{tab:gen_sen-full} in the Appendix for sentences from the other two corpora.}
    \label{tab:gen_sen}
    \end{table*}

==> preamble_acronyms.tex <==
% A
\newacronym{ADVI}{advi}{automatic differentiation variational inference}
\newacronym{AR}{a{\small\&}r}{augment and reduce}

% B
\newacronym{BBVI}{bbvi}{black-box variational inference}

% C
\newacronym{CDF}{cdf}{cumulative distribution function}
\newacronym{CS-EFE}{cs-efe}{context selection for exponential family embeddings}
\newacronym{CTM}{ctm}{correlated topic model}

% D
\newacronym[\glslongpluralkey={deep exponential families}]{DEF}{def}{deep exponential family}
\newacronym{DMIS}{dmis}{deterministic multiple importance sampling}

% E
\newacronym{EFE}{efe}{exponential family embeddings}
\newacronym{ELBO}{elbo}{evidence lower bound}
\newacronym{EM}{em}{expectation maximization}

% G
\newacronym{GNTS}{gn-ts}{gamma-normal time series model}
\newacronym{G-REP}{g-rep}{generalized reparameterization}

% H
\newacronym{HMC}{hmc}{{H}amiltonian {M}onte {C}arlo}

% K
\newacronym{KL}{kl}{{K}ullback-{L}eibler}

% L
\newacronym{LDA}{lda}{latent {D}irichlet allocation}

% M
\newacronym{MAP}{map}{\emph{maximum a posteriori}}
\newacronym{MCMC}{mcmc}{{M}arkov chain {M}onte {C}arlo}
\newacronym{MF}{mf}{matrix factorization}
\newacronym{MIS}{mis}{multiple importance sampling}

% O
\newacronym{OBBVI}{o-bbvi}{overdispersed black-box variational inference}
\newacronym{OVE}{ove}{one-vs-each}

% S
\newacronym{SIVI}{sivi}{semi-implicit variational inference}
\newacronym{SVI}{svi}{stochastic variational inference}

%U
\newacronym{USIVI}{uivi}{unbiased implicit variational inference}

% V
\newacronym{VAE}{vae}{variational autoencoder}
\newacronym{VEM}{vem}{variational expectation maximization}
\newacronym{VI}{vi}{variational inference}


